Accelerating Path Planning for Autonomous Driving with Hardware-Assisted Memoization

Path planning for autonomous driving with dynamic obstacles poses a challenge because it needs to perform a higher-dimensional search (with time-dimension) while still meeting real-time constraints. This paper proposes an algorithm-hardware co-optimization approach to accelerate path planning with high-dimensional search space. First, we reduce the time for a nearest neighbor search and collision detection by mapping nodes and obstacles to a lower-dimensional space and memoizing recent search results. Then, we propose a hardware extension for efficient memoization. The experimental results on a modern processor and a cycle-level simulator show that the hardware-assisted memoization significantly reduces the execution time of path planning.

==> 2020-robot-accelerator 2/challenge.tex <==
%\section{Challenges}\label{sec:challenge}

%\section{Analysis}\label{sec:analysis}





\begin{comment}

We are focusing on sampling-based motion planning algorithm for high safety-assurance 
applications like autonomous driving and robot arms for surgery. \cite{sozzi2019dynamic}The major 
challenges 
facing these motion planning problems is the increased search space, and low performance 
improvement bring about by the traditional LSH-based scheme. Besides, as motion planning 
algorithm is constantly evolving, a hardware accelerator needs to have enough 
programmability/flexibility in adapting to different algorithms.

\end{comment}

\begin{comment}
\subsection{Increased Search Spaces}


A dynamic obstacle has different positions at different times. As a result, instead of being 
represented as a single point in workspace, it has to be represented as a curve in the 
workspace-time \cite{schwesinger2015fast} space where the time is serving as an additional 
dimension.

Another dimension that needs to be considered is the different predictions of dynamic 
obstacles. For example, at a crossroad, an incoming vehicle might be going straight, turning 
left, or turning right. The motion planner needs to take each of the scenario separately, and 
the solution needs to consider the risk and benefit of all these scenarios. Thus, an additional 
discrete dimension is needed.



Third, due to the measurement error, the motion planning algorithm will need to 
probablistically consider the collision. Monte-Carlo based collision calculation has been 
widely used in motion planls -lrtning due to its accuracy compared to simplified belief-propagation 
based motion planning. This means an additional dimension over different samples.

The increased dimensionality makes it significantly harder to meet the deadline that is 
required for high-assurance motion planning. Contigency  planning\cite{hardy2013contingency} which 
is a work that systematically considers these scenarios, barely meets the 
computation deadline of 100ms for autonomous driving. Though GPU may also help in some 
of the scenario \cite{ichter2017robust} and other algorithmic approaches have been 
proposed, there lacks a comprehensive solution that addresses these challenges.


 
%dynamic obstacles, multiple scenarios

\end{comment}
\begin{comment}

\subsection{Programmability}

% existing accelerator lacks programmability
% simple CPU/GPU is too expensive

Due to the wide reach of internet connectivity, software or firmware update is more 
convenient than before. As a result, remote update has been used in autonomous 
driving and robotic products to enable new functionality that is not readily available at the 
time of delivery. For hardware accelerators, upgradability to the algorithm is essential since 
the road conditions, traffic laws are evolving fast, and today's state-of-the-art motion 
planning algorithm may not be the best for tomorrow's needs. Cars and robots usually last 
around ten years, and the accelerator needs to be able to adapt to the potential new 
algorithms over the years. However, it is hard to strike a balance between the general 
programmability and performance, and energy efficiency.  CPU and GPU provides good 
programmability, but it is hard to achieve the performance and energe-efficiency 
simulataneously. Existing motion planning accelerators, on the other hand, make very 
specialized optimization which results in lack of programmability.  

\end{comment}

==> 2020-robot-accelerator 2/design.tex <==
\section{Approach}\label{sec:design}
 
 %\subsection{Planning Algorithm for Acceleration}
 
%We describe the design of our memorization approach for dynamic obstacle path planning in this 
%section.

%We describe our acceleration approach for path planning with dynamic obstacles in this section.

\noindent{\bf Handling Dynamic Obstacles. }
Let us consider path planning for an autonomous vehicle on a 2D plane. At different times, 
obstacles will be at different positions on the 2D plane.  A dynamic obstacle in a 2D plane becomes a 
set 
of obstacles 
whose coordinates in the 3D space can be described by $(x, y, t)$. We can effectively regard 
the 2D 
planning problem with  dynamic obstacles as a 3D planning problem.
However, the time dimension is different from a normal spatial dimension and introduces 
an additional 
constraint. Since time only goes in one direction, for any two nodes $(x_i, y_i, t_i)$ and 
$(x_j, y_j, t_j)$ on a path P where $i < j$, we must guarantee $t_i < t_j$. The additional constraint is 
enforced when selecting nearest neighbors in RRT. 

\begin{comment}

  \begin{figure}[h]
	\centering
	\includegraphics[width=0.8\linewidth]{fig/dyn}
	\caption{Comparison of the dimensions of the search space of path planning with  a static 
	obstacle (left) and a 
	dynamic obstacle (right).}\label{fig:dyn}
	\vspace{-0.25cm}
\end{figure}
\end{comment}


\noindent{\bf Software-based Memoization. }
We use memoization to reduce the total execution time of path planning. 
In traditional sampling-based planning, 
a large portion of the execution time is spent on finding the nearest neighbor (NN) and detecting collisions.  To 
accelerate these 
 procedures, we memoize the recently accessed nodes and the collision state so that some of 
 the similar queries  can be 
 skipped. 
 Figure~\ref{fig:flow} shows the high-level flow of our approach. In the 
baseline RRT, the time-consuming nearest neighbor search and collision detection are performed 
for all iterations. 
However, we use an small-size data storage named {\em Morton store} (named after Morton space-filing 
curve \cite{open2017discrete}) to 
memoize the key 
information from 
baseline nearest neighbor search and collision detection. For each iteration, we always check the Morton store first 
to 
opportunistically skip the time-consuming baseline NN search and collision detection.

  \begin{figure}[h]
  		\vspace{-0.5cm}
	\centering
	\includegraphics[width=0.6\columnwidth]{fig/flow}
	\vspace{-0.25cm}
	\caption{The baseline (blue arrows) and proposed (orange arrows) planning 
	flow.}\label{fig:flow}
			\vspace{-0.25cm}
\end{figure}
%\vspace{-0.25cm}

The  Morton store works as follows.
We first calculate the Morton codes $M_n$  and $M_o$ for the coordinates of both tree nodes 
$X_n=(x_n, y_n, t_n)$ 
and 
obstacles $X_o=(x_o, y_o, t_o)$. 
Morton code projects point $(x, y, t)$  from 3D space onto a 1D curve, while maintaining spatial 
locality ($x$, $y$, $t$ are represented as 32-bit integers).
The Morton codes $M_n$  and $M_o$  are 64-bit numbers and are used as the tags for the 
corresponding nodes and 
obstacles. 
To adjust the projection granularity, we mask $k$ least significant bits of the Morton code 
\begin{equation}
	M_n' \gets M_n\; \texttt{\&} \; \underbrace{1...1}_{(64-k)\; bits}\underbrace{0...0}_{k\; bits}
\end{equation}


%To 
%adjust the granuarity, we apply a mask on the tag to filter out the MSB, in general, the less MSBs being 
%kept, the larger the granuarity. 

The pseudocode for the Morton-store based acceleration approach is shown in Algorithm~\ref{alg:cap}.
For each iteration we first generate  a new random node (Line~2). Then we calculate its masked Morton 
code and 
search for entries with matching Morton codes in the Morton store (Line~3). If there is no match in 
the Morton store,  we perform the baseline nearest neighbor search using 
kdtree (Line~4). Then we perform the ``steer'' operation to find a node along the direction of 
$X_{rand}$ but with unit distance to $X_{nearest}$.  For 
collision detection, we also check the Morton store first (Line~8). 
If the result indicates that it is not NO\_COLLISION state (could be COLLISION state or a miss), we do 
more 
time-consuming baseline detailed 
collision detection (Line~9). After that, we update the 
Morton store (Line~11) and the baseline tree (Line~12-14).
The solution path has to perform exact collision detection for each segment to make sure the path 
is indeed safe (NO\_COLLISION). Compared with the time saved by not performing exact collision detection 
using the Morton store, the 
solution checking overhead is negligible. The time complexity of the algorithm is 
$O(N\cdot(\alpha \cdot log N+\beta\cdot  log L))$ where $N$ is the number of nodes in the tree, $L$ is 
the 
number of obstacles, and $\alpha$, $\beta$ are probabilities Line~8 and Line~12 are taken, respectively 
($0< 
\alpha, \beta\leq 1$). For normal RRT without using the Morton store, we have $\alpha, \beta = 
1$.



\begin{algorithm}
	\scriptsize
	\caption{RRT with Morton code-based memoization}\label{alg:cap}
	\begin{algorithmic}[1]
		\While {$X_{goal}$ not reached}
		\State {$X_{rand} \gets  rand() $}
		\If {$X_{nearest}\gets morton\_nn(X_{rand}) == \emptyset $}
		\State {$X_{nearest}\gets nearest(X_{rand}) $}
		\EndIf
		\State {$X_{new}\gets steer(X_{nearest}, X_{rand}) $}
		\State {$state\gets morton\_collision(X_{new}, X_{nearest})$}
		\If {$state !=NO\_COLLISION$}
		\State {$state\gets collision(X_{new})$}
		\EndIf
		\State {$morton\_update(state, X_{new})$}
		\If {$collision(X_{new}, X_{nearest})==NO\_COLLISION $ }
		\State {$nn.add(X_{new})$}
		\EndIf
		\EndWhile
	\end{algorithmic}
\end{algorithm}

%\vspace{-0.25cm}

%There are three additional parameters, the number of tags in the array, the number entries of for each 
%tag, and the threshold. 

\noindent{\bf Hardware-Assisted Memoization. } The software-based Morton store reduces the 
execution time significantly by skipping 
 time-consuming baseline NN search and collision detection, and it 
 can be further accelerated by hardware-assisted memoization. Since Morton code calculation and 
 matching is processed by 
 iterating all the existing Morton codes sequentially in software, it can take multiple instructions. 
  To estimate how 
 many dynamic instructions
 the Morton store takes, we use Valgrind \cite{valgrind} to count the 
 number of dynamic intructions of 
 the Morton store lookups and updates. 
 \begin{figure}[h]
 	\centering
 	\includegraphics[width=0.99\linewidth]{fig/morton}
 	\caption{Percentage of dynamic instruction count of the Morton store lookups and 
 	updates, geomean is shown in the last column. }\label{fig:morton}
 	\vspace{-0.25cm}
 \end{figure}
 
 Figure~\ref{fig:morton} shows the profiled results of different testcases with different map edge 
 length,  timesteps, and number of 
 dynamic obstacles. The geomean shows that
 Morton store-related dynamic instruction count accounts for ~27\% of the maximum total dynamic 
 instructions, and in the 
 worst case, it 
 can be 
 more than 45\% of the total number of dynamic instructions. 
  However, with hardware-assisted memoization, the dynamic instruction counts can be reduced 
  dramatically. 
We can use content-addressable memory for the Morton store lookup and update
 directly in hardware to reduce the dynamic instruction count and the correspondingly the execution 
 time.
 
 \begin{figure}
 	\vspace{-0.25cm}
	\centering
	\includegraphics[width=0.99\linewidth]{fig/mem}
	\vspace{-0.75cm}
	\caption{HW-based Morton store implemented by content-addressable 
	memory.}\label{fig:mem}
		\vspace{-0.25cm}
\end{figure}
%\vspace{-0.25cm}

% \vspace{0.25cm}
\begin{figure}[h]
	\centering
%	\vspace{-0.25cm}
	\includegraphics[width=0.6\linewidth]{fig/arch}
	\vspace{-0.25cm}
	\caption{Overall architecture with Morton store.}\label{fig:arch}
	\vspace{-0.5cm}
\end{figure}
%\vspace{-0.25cm}

 
 The hardware-based Morton store  is implemented by a fully-associative content-addressable 
 memory 
 whose memoryline size is 64 bytes. Each line can store eight 8-byte addresses of RRT nodes. 
 Since these nodes are allocated on the stack, the MSBs are always 0 in our settings, and 
 we use the most significant 8 bits of the address to indicate whether there is a collision or not. Figure~\ref{fig:mem} 
 shows an example of the hardware Morton store implemented in content-addressable memory
 The tagstore keeps the 
 Morton codes, and each row contains the state (collision/no collision) information as well as the 
 addresses of the nodes. For collision state, as long as there is one state that indicates collision among all states in 
 one memoryline, the output will be a collision. 
 %We do not explicitly store the addresses of the obstacles in the Morton store.
 
 

 The content-addressable memory is connected directly to the CPU, as shown in
Figure~\ref{fig:arch}.  On a hit, the 
 corresponding memoryline used for extracting collision state or a node address is processed. 
 On a read miss, nothing is modified in the Morton store. On a write miss, the oldest 
 referenced memoryline is evicted.
 In order to access this content-addressable memory in software and provide flexibilty to different planning 
 algorithms, we define the following ISA 
 extensions: \texttt{morton\_update}, \texttt{morton\_col} and \texttt{morton\_nn} which are listed in 
 Table~\ref{tab:isa}.
 \texttt{morton\_update} takes in the coordinates of a node and its collision state and updates this 
information in the Morton store. \texttt{morton\_col} takes in the coordinates of a 
node, look it up in the content-addressable memory and decides whether there is a collision. 
\texttt{morton\_nn} finds the memory address of the approximate nearest 
neighbor in the Morton store by looking up entry with the same Morton code.
In this work, we use these instructions to accelerate RRT. However, it can also be used in other 
sampling-based planning 
algorithms such as PRM.

  
 \begin{table*}
 	\footnotesize
 	%\scriptsize
 	\centering
 	\caption{ISA interface for Morton store.}\label{tab:isa}
 	 	\vspace{-0.25cm}
 	\begin{tabular}{|l|l|l|}
 		\hline
 		\bf ISA Instruction & \bf Operation\\ \hline\hline
 		\texttt{morton\_update <x|y>, <t>, <addr>} &     Update a node with coordinate $(x,y, t)$ and 
 		memory address \texttt{addr} in Morton store \\ \hline
 		\texttt{morton\_col <x|y>, <t>, <st>}&    Check whether there is a collision for the node $(x,y,t)$ 
 		using 
 		Morton 
 		store, returns result in \texttt{st} \\ \hline
 		\texttt{morton\_nn <x|y>, <t>, <addr> }& Find an approximate near neighbor of the node  $(x,y, 
 		t)$, returns the 
 		address in \texttt{addr} \\ \hline
 		
 	\end{tabular}
 	\vspace{-0.25cm}
 \end{table*}
 
 
 


==> 2020-robot-accelerator 2/discussion.tex <==
\section{Discussion}\label{sec:discussion}



Our approach is inspired by two key ideas: pruning, and content-addressable 
memory-based acceleration.
Pruning is inspired by Pan\cite{pan2016fast}, which uses location sensitive hash 
(LSH) for pruning exact collision detection computation. 
However, the proposed software optimization with the Morton codes differs in several 
ways. 
First, we are focusing on autonomous driving scenario, which usually only have 
limited degrees of 
freedom, in these case, the benefit of using multiple hash functions to reduce 
the dimension is 
marginal.
Instead, we use the space-filling curve. However, in this case, precise matching of  
Morton code is 
hard, and we remove some LSBs and only use MSBs  
of the Morton code in order to increase the probability of a Morton 
store hit.
Using one table instead of multiple LSHs also makes an efficient hardware implementation possible. 

 \begin{table*}[h]
%	\footnotesize
\centering
\scriptsize
%\footnotesize
	\caption{Comparison with existing works.}\label{tab:compare}
	\begin{tabular}{|l|| l|l|l|l|l|l| l|}
		\hline
		work &  implementation & encode  &  reported improvement  & 
		algorithm & dynamic &accelerate& accelerate\\ 
		& & & over SW& flexibility& obstacles &tree search& collision detection\\ \hline\hline
		\cite{pan2016fast} &  software & LSH  & 1.46X   &  yes& no & no& yes \\ \hline
		\cite{yang2020accelerating} & accelerator & RENE \cite{bremler2018encoding}  &  
		235X&  no& no &yes&yes \\ \hline
		 \cite{kim2017brain} & processor & Zobrist \cite{zobrist1990new} & 8.63X & 
		 no & 
		 no&yes& no\\ \hline
		this work &  ISA extension &   Morton & 8X &  yes &yes&yes&yes\\ \hline
	\end{tabular}
    \label{tab:comparion}
	\vspace{-0.5cm}
\end{table*}

 The content-addressable memory for path planning is inspired by 
 \cite{yang2020accelerating}. However, our work is different from it in several ways. 
 First, our work has just one 
 unified Morton store that is used  for both collision detection and nearest neighbor 
 search, while 
 the previous work uses 
 two separate stores. Second, our work is designed as an ISA extension to a 
 normal processor, 
 and adapt to 
 different algorithms, while the previous work \cite{yang2020accelerating} is limited
 to a fixed algorithm with the size of 
 the 
 problem that can 
 fit into the ternary-CAM available on chip. 
 \cite{kim2017brain} also uses CAM for path planning algorithms. 
 However, the it only targets the A* search algorithm, not sampling-based path 
 planning. 
 Also, this previous work cannot completely 
 skip the tree search and does not explicitly accelerate collision detection.
 Table~\ref{tab:compare} summarizes 
 the major differences between our work and the related work on pruning and CAM-based acceleration. 
% Our work strikes a 
% good balance in performance and flexibility.
 
 

 
 
 
\begin{comment}

\subsection{Location Sensitive Hash}

As mentioned, new concerns in motion planning problems, including dynamic 
obstacles, 
multiple paths of obstacles, and probabilistic collision \cite{hardy2013contingency}, 
have 
significantly increase the dimensionality and the number of samples in a 
sampling-based 
motion planning algorithms. LSH-based method \cite{pan2016fast} is an effective 
way to 
accelerate the 
search in high-dimensional space. Usually, LSH have multiple hashtables with 
different hash 
functions. Points that are close to each other are likely to be mapped to the same 
bucket in 
one or more hashTables. LSH is efficient in search for the nearest neighbors, which 
is needed 
for a sampling-based motion planning algorithm like RRT \cite{guo2018foggycache}. 
LSH 
has also been used for collision checking in motion-planning algorithms 
\cite{pan2011fast} on the assumption that collision checking takes most of 
	the 
computation time in motion planning. LSH is a good primitive for accelerating motion 
planning algorithms.



\subsection{Existing LSH Scheme}

Though LSH has been used with existing motion planning for nearest neighbor 
search or 
collision detection in software. Only modest improvement has been observed 
because unoptimized 
hash table may consume significant hardware resource. Hash table can be 
hardware friendly since on-chip memory like caches can be used to accelerate the 
table 
lookup by preventing direct access to the main memory similar to how translation 
lookup 
buffer can help accelerating pagetable lookup. However, on-chip memory has 
limited sizes 
that might not be able to cache the entire table and it remains unclear what is the 
proper size 
of the caches.  Even though there are existing works on building cache-friendly 
motion 
planning algorithms, there have not been any works on software-hardware 
co-optimized 
LSH. 

%LSH only accelerates collision checking, but with increased dimensions, tree 
%traversal is also important

% existing LSH does not leverage the HW 


Location sensitive hash (LSH) can reduce the computation time in a high dimensional 
space [cite]. LSH is a class of hash function that maps spatially remote coordinates 
to hash values with larger distances. A formal definition of LSH can be found at 
[cite]. Using LSH, similar queries (searches) in the high dimensional space can be 
accessed quickly by directly looking up the hash table which stores queries with 
similar LSH values. LSH has also been used separately for collision detection in the 
path planning algorithm, with the assumption that in traditional path planning 
algorithm, collision checking, rather than tree traversal takes most of the time. 
However, in high dimensional case with more obstacles, and when we apply BVH to 
prune unnecessary collision checkings, we observe that the collision checking and 
tree traversal are equally important in the computation time. 
%An LSH-based scheme that accelerates both collision checking and tree traversal 
%is needed in these 
%scenarios.
Besides, most of the existing LSH-based scheme are purely software-based 
\cite{pan2011fast} without 
leveraging hardware structures that could be used in a accelerator structure. As a 
result, existing 
approach \cite{pan2016fast} for accelerating collision checking only bring about less 
than 30\% 
performance improvement. 

\end{comment}


==> 2020-robot-accelerator 2/evaluation.tex <==

\section{Evaluation}\label{sec:evaluation}
\begin{comment}
In this section, we evaluate the effectiveness of the proposed memoization scheme based on  
the Morton code for both software and hardware implementations.
\end{comment}

%First, we describe the testcases we use for our 
%evaluation of path planning with dynamic obstacles. 
%Then, we show our evaluation 
%results for software and hardware-assisted 
%Morton store.

\noindent{\bf Synthetic Test Cases.} Each synthetic test case is defined on a square 
map, with dynamic obstacles running on it. The synthetic 
test cases are characterized 
by three 
parameters, i.e., the number of dynamic obstacles, the edge length of the square map, and 
the 
number of time steps. The solution path should start at $(0,0)$ and destination is $(l,l)$ 
where $l$ is the edge length of the square map.
We randomly generate the starting and ending locations of the obstacles at the 
beginning and the 
ending of the simulation period. The intermediate positions of the obstacles are  linearly 
interpolated. Figure~\ref{fig:3drrt} shows an example of the 
test case with 5 
dynamic obstacles, the edge length of 100, and 20 time steps. The solution path from (0,0) to 
(100,100) is 
marked in blue.


  \begin{figure}[h]
	\centering
	\includegraphics[width=0.9\linewidth]{fig/3drrt}
	\caption{A test case with 5 dynamic obstacles, edge length 100, and 20 
	time steps. The solution path is shown in blue.}\label{fig:3drrt}
\vspace{-0.25cm}
\end{figure}
%\end{comment}

\begin{comment}
\begin{figure}
	\vspace{-0.25cm}
	\centering
	%\includegraphics[width=0.95\textwidth]{fig_source/svt.pdf}
	%\caption{Number of particles for a straight route and a route with a turn.}
	%\label{fig:svc}
	\begin{minipage}[t]{0.45\linewidth} 
		\centering
	\includegraphics[width=0.95\linewidth]{fig/3drrt}
\caption{A testcase with 5 dynamic obstacles, edge length 100, and 20 
	timesteps.}\label{fig:3drrt}
	\end{minipage}  
	\hspace{0.25cm}
	\begin{minipage}[t]{0.45\linewidth}
		\centering
	\includegraphics[width=0.95\linewidth]{fig/3drrt2}
\caption{A testcase with 5 dynamic obstacles, edge length 100, and 20 
	timesteps.}\label{fig:3drrt2}
	\end{minipage}
	\vspace{-0.25cm}
\end{figure}
\end{comment}
The number of obstacles determines the difficulty of the path planning problem. 
In general, with more 
obstacles, it takes more time to find a safe path and the length of the path 
may also be longer 
because more space is occupied by the obstacles.
The edge length of the map and the number of time steps mainly increase the execution 
time for path planning. On the 
other hand, 
a longer edge length and more time steps will provide more accurate solutions with 
more 
intermediate points along the 
path.



\noindent{\bf Software Performance Evaluation. }
We evaluate the  software-based Morton store  on a desktop with a 3.4GHz Intel i7-6700 
CPU and 16GB DDR4 memory at 2133MHz.
%The configuration of the processor is shown in Table~\ref{tab:proc}.
The baseline RRT algorithm is implemented in C++.  The baseline nearest neighbor 
search is based on kd-tree  \cite{kdtree}.
%http://nuclear.mutantstargoat.com/sw/kdtree/.
We use libmorton \cite{libmorton18} 
for  Morton code calculation. 

\begin{comment}

\begin{table}
	\scriptsize
	\centering
		\caption{Processor configuration.}\label{tab:proc}
	\begin{tabular}{|l|l|}
		\hline
		Name &  Intel i7-6700 CPU  3.40GHz\\ \hline
		Core &   SkyLake  \\ \hline
		L1-i &   32KB, 8-way \\ \hline
		L1-d&   32KB, 8-way \\ \hline
		L2& 256KB , 4-way \\  \hline
		L3&  8MB\\ \hline
		Memory& 16GB, DDR4@2133MHz\\ \hline
	\end{tabular}

\end{table}

\end{comment}

  \begin{figure}
	\centering
	\vspace{-0.5cm}
	\includegraphics[width=0.99\linewidth]{fig/exectime}
	\caption{Execution time of the baseline and the software Morton 
		store (software on Intel i7), geomean is shown in the last column.}\label{fig:exectime}
	\vspace{-0.25cm}
\end{figure}

We simulate 12 configurations with the map edge length in \{100, 200\}, the number of time steps in 
\{10,100\}, and
the number of obstacles in \{5, 10, 20\}. 
We compare the total execution time of the baseline RRT and the RRT with the software Morton-store 
(sw-morton). We choose  $k=18$ least significant bits to mask.
For each configuration, we randomly generate 10 different test cases.  As the 
algorithm is a 
randomized 
algorithm, for each test case, we repeat each experiment 10 times and show the 
average 
execution time.
Figure~\ref{fig:exectime} shows the execution time. On average, the software Morton 
%store-based path planning reduces the execution time by 51\% compared to the baseline RRT.
store-based path planning has 1.96$\times$  performance improvement over the baseline RRT.


%We also compare the impact of the impact of the size of the array, and mask and 
%number of pointers, 
%the results are shown in Figure~\ref{fig:}. 
%In general, larger arrays, more number of nodes for each tags are better at 
%reducing 
%the total execution 
%time.

\noindent{\bf Hardware Evaluation. }
The proposed hardware-assisted approach uses the content-addressable memory for 
a fast look-up and update of the recently-accessed tree nodes for the nearest neighbor search and  
collision detection.
We evaluate the performance of this hardware-based Morton store using gem5 simulator 
\cite{Binkert11thegem5}. The simulator configuration is shown in 
Table~\ref{tab:gem5}. We implemented a HW Morton store and a customized port 
between a CPU and a HW Morton store  
for the look-up and update in gem5. We choose $k=18$ least significant bits to mask.

\begin{table}
	\vspace{-0.25cm}
	\scriptsize
	\centering
	\caption{gem5 configuration.}\label{tab:gem5}
		\vspace{-0.25cm}
	\begin{tabular}{|l|l|}
		\hline
\bf Core &   Simple Timing CPU @ 2GHz  \\ \hline
\bf L1-i&   32KB, 4-way, latency=2 cycles \\ \hline
\bf L1-d&   32KB, 8-way, latency=2 cycles \\ \hline
\bf Morton Store& 32KB, fully-associative, memoryline=64 bytes, latency=2 cycles \\ \hline
\bf L2& 256KB , 8-way, latency=20 cycles \\  \hline
\bf L3&  8MB,16-way, latency=20 cycles\\ \hline
\bf Memory& 4GB, DDR3@1600MHz \\ \hline
	\end{tabular}
\vspace{-0.25cm}
\end{table}

\begin{comment}
\begin{figure}
	%\vspace{-0.25cm}
	\centering
	%\includegraphics[width=0.95\textwidth]{fig_source/svt.pdf}
	%\caption{Number of particles for a straight route and a route with a turn.}
	%\label{fig:svc}
	\begin{minipage}[t]{0.45\linewidth} 
		\centering
		\includegraphics[width=0.99\textwidth]{fig/baseline2}
		\vspace{-0.5cm}
		\caption{Solution path on the map by baseline RRT with length 175.}
		\label{fig:baseline}
		\vspace{-0.25cm}
	\end{minipage}  
	\hspace{0.25cm}
	\begin{minipage}[t]{0.45\linewidth}
		\centering
		\includegraphics[width=0.99\textwidth]{fig/hw-morton2}
		\vspace{-0.5cm}
		\caption{Solution path by the HW-based Morton store with length 217.}
		\label{fig:hw-morton}
		\vspace{-0.25cm}
	\end{minipage}
	\vspace{-0.25cm}
\end{figure} 
\end{comment}


\begin{figure}
			\centering
	\includegraphics[width=0.45\columnwidth]{fig/baseline2}
%	\vspace{-0.5cm}
	\caption{Solution path on the map by baseline RRT with length 175.}
	\label{fig:baseline}
	\vspace{-0.25cm}
\end{figure}

\begin{figure}
		\centering
\includegraphics[width=0.45\columnwidth]{fig/hw-morton2}
%\vspace{-0.5cm}
\caption{Solution path by the HW-based Morton store with length 217.}
\label{fig:hw-morton}
\vspace{-0.25cm}
\end{figure}


\begin{figure}
		\centering
	%	\vspace{-0.5cm}
\includegraphics[width=0.99\linewidth]{fig/time}
\vspace{-0.5cm}
\caption{Execution time comparison (gem5 simulation results), geomean is shown in the last column. 
}\label{fig:time}
\vspace{-0.5cm}
\end{figure}


\begin{figure}
	\centering
%	\vspace{-0.25cm}
	\includegraphics[width=0.99\linewidth]{fig/length}
	\vspace{-0.5cm}
	\caption{Solution length comparison, geomean is shown in the last column. }\label{fig:length}
	\vspace{-0.5cm}
\end{figure}


\begin{comment}

\begin{figure*}
	\vspace{-0.25cm}
	\centering
	%\includegraphics[width=0.95\textwidth]{fig_source/svt.pdf}
	%\caption{Number of particles for a straight route and a route with a turn.}
	%\label{fig:svc}
	\begin{minipage}[t]{0.49\linewidth} 
		\centering
		\includegraphics[width=0.99\linewidth]{fig/time}
		\vspace{-0.25cm}
		\caption{Execution time comparison (simulation results).}\label{fig:time}
	\end{minipage}  
	%	\hspace{0.5cm}
	\begin{minipage}[t]{0.49\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{fig/length}
		\vspace{-0.25cm}
		\caption{Solution length comparison.}\label{fig:length}
	\end{minipage}
	%\vspace{-0.5cm}
\end{figure*} 

\end{comment}

We use the same 12 configurations that are used in the software evaluation in the 
previous subsection.
Figure~\ref{fig:time} shows the execution time of the baseline, the software-based Morton  
store (sw-morton)
 and the hardware-based Morton (hw-morton) store based on gem5 simulation.
The performance improvements over the baseline are 2.28$\times$  for software-based Morton store 
(which is 
similar to 1.96$\times$  in software simulation using Intel i7 processor.) and 8$\times$  for 
the hardware-based Morton store on average. 
For the best 
 configuration, the performance is improved by 6.74$\times$  and 56.3$\times$  for software 
 and 
 hardware Morton stores,
 respectively.
Figure~\ref{fig:length} shows the solution path lengths for the baseline, the software-based 
Morton store and 
the hardware-based Morton store. The average solution length of the software Morton 
and hardware 
Morton stores  
are 1.42$\times$  and 1.65$\times$  higher than that of the baseline solution. This is due to the fact 
that 
the SW or HW Morton store can only find approximate nearest neighbor instead 
of the exact nearest neighbor. Thus, the solution path may fluctuate more compared to the baseline.
As shown in Figure~\ref{fig:hw-morton}, around position $(80, 80)$ of the map, the path 
given by the HW-based Morton store moves back and forth before 
reaching $(100, 100)$, which increases the solution length compared to the baseline 
solution shown in Figure~\ref{fig:baseline}. Such path can use refinement 
\cite{alterovitz2011rapidly} 
to reduce the overall length.

%\vspace{-0.5cm}




\noindent{\bf Commonroad Evaluation.} To demonstrate the effectiveness of the proposed method on 
realistic scenarios, we use one example (\texttt{USA\_US101-20\_1\_T\_1}) shown in 
Figure~\ref{fig:usa_us101} containing dynamic 
obstacles from the Commonroad 
\cite{althoff2017commonroad} benchmarks, whose scenarios are partly recorded from real traffic. The 
execution time and solution path lengths are shown in Figure~\ref{fig:usa_us101_perf}, which confirms 
effectiveness in reducing the execution time.

%\begin{comment}


\begin{table*}[h]
	%	\footnotesize
	\centering
	\scriptsize
	%\footnotesize
	\caption{Comparison with existing works.}\label{tab:compare}
	\vspace{-0.25cm}
	\begin{tabular}{|l|| l|l|l|l|l|l| l|}
		\hline
		work &  implementation & indexing  &  reported improvement  & 
		algorithm & dynamic &accelerate& accelerate\\ 
		& & method & over SW& flexibility& obstacles &tree search& collision detection\\ 
		\hline\hline
		\cite{pan2016fast} &  software & LSH  & 1.46$\times$    &  yes& no & no& yes \\ \hline
		\cite{yang2020accelerating} & accelerator & RENE \cite{bremler2018encoding}  
		&  
		235$\times$ &  no& no &yes&yes \\ \hline
		\cite{kim2017brain} & processor & Zobrist \cite{zobrist1990new} & 8.63$\times$  & 
		no & 
		no&yes& no\\ \hline
		this work &  ISA extension &   Morton & 8$\times$  &  yes &yes&yes&yes\\ \hline
	\end{tabular}
	\label{tab:comparion}
	\vspace{-0.25cm}
\end{table*}

\begin{figure}
	%\vspace{-0.25cm}
	\centering
	%\includegraphics[width=0.95\textwidth]{fig_source/svt.pdf}
	%\caption{Number of particles for a straight route and a route with a turn.}
	%\label{fig:svc}
	\begin{minipage}[t]{0.41\linewidth} 
		\centering
		\includegraphics[width=0.65\linewidth]{fig/usa_us101}
		\vspace{-0.25cm}
		\caption{\texttt{USA\_US101-20\_1\_T\_1} from Commonroad 
			benchmarks. Blue blocks are moving obstacles, grey stripes are the lanes, green arrow is the 
			initial 
			position and yellow dot is the destination.}\label{fig:usa_us101}
		\vspace{-0.25cm}
	\end{minipage}  
	\hspace{0.25cm}
	\begin{minipage}[t]{0.49\linewidth}
		\centering
		\includegraphics[width=\textwidth]{fig/usa_us101_perf}
		\vspace{-0.25cm}
		\caption{Execution time and solution length comparison of   
			\texttt{USA\_US101-20\_1\_T\_1}, sw- and hw-morton achieves 4.3$\times$  and 35$\times$  
			execution time 
			reductions.}
		\label{fig:usa_us101_perf}
		\vspace{-0.25cm}
	\end{minipage}
	\vspace{-0.25cm}
\end{figure} 

%\end{comment}

\begin{comment}
\begin{figure}
		\centering
\includegraphics[width=0.4\columnwidth]{fig/usa_us101}
\vspace{-0.25cm}
\caption{\texttt{USA\_US101-20\_1\_T\_1} from Commonroad 
	benchmarks. Blue blocks are moving obstacles, grey stripes are the lanes, green arrow is the 
	initial 
	position and yellow dot is the destination.}\label{fig:usa_us101}
\vspace{-0.25cm}
\end{figure}

\begin{figure}
		\centering
\includegraphics[width=0.6\columnwidth]{fig/usa_us101_perf}
\vspace{-0.25cm}
\caption{Execution time and solution length comparison of   
	\texttt{USA\_US101-20\_1\_T\_1}, sw-Morton and hw-Morton achieves 4.3X and 35X execution time 
	reductions.}
\label{fig:usa_us101_perf}
\vspace{-0.5cm}
\end{figure}
\end{comment}



\begin{comment}

   \begin{figure}[h]
	\centering
	\includegraphics[width=0.95\linewidth]{fig/time}
	\caption{Execution time comparison.}\label{fig:time}
\end{figure}

   \begin{figure}[h]
	\centering
	\includegraphics[width=0.95\linewidth]{fig/length}
	\caption{Solution length comparison.}\label{fig:length}
\end{figure}

\end{comment}

%\subsection{Quality of Solutions}





==> 2020-robot-accelerator 2/implementation.tex <==
%\section{Implementation}\label{sec:implemenation}

==> 2020-robot-accelerator 2/intro.tex <==
\section{Introduction}
% no \IEEEPARstart
%This demo file is intended to serve as a ``starter file''
%for IEEE conference papers produced under \LaTeX\ using
%IEEEtran.cls version 1.7 and later.
% You must have at least 2 lines in the paragraph with the drop letter
% (should never be an issue)
%I wish you the best of success.

%\hfill mds
 
%\hfill January 11, 2007

%Motion planning is widely used in the emerging applications including autonomous 
%driving, remote 
%healthcare, robot manipulator, and unmanned aerial vehicles. Due to the increasing 
%accuracy and 
%safety requirements, motion planning algorithms are becoming increasingly 
%complex, and as a result, it 
%takes significant amount of computation time. 




Path planning for autonomous driving faces challenges including
strict real-time constraints as well as  dynamic obstacles.
First, in autonomous driving, path planning can take 100 $ms$  on average on a 
commercial  autonomous driving development platform \cite{yu2020building} like 
Baidu Apollo, while  the safety 
requirement assumes the 
sensor-to-actuator latency must be less than 100 $ms$ \cite{lin2018architectural} to ensure 
the 
responsiveness.  
Second, modern autonomous vehicles have to deal with 
dynamic obstacles. In real-world streets, there are other vehicles moving at high 
speed, and there are pedestrians walking at low speed. Path planning algorithm has 
to deal 
with these moving objects and avoid collisions. The vehicles
have to take into account the locations of the obstacles at different timesteps.
Recent studies on path planning algorithms 
such as PUMP \cite{ichter2017robust} and contingency 
planning \cite{hardy2013contingency} consider dynamic obstacles. However, it  
could take as long as 500 $ms$ to compute 
a path in these scenarios on a CPU. 
Even on a GPU, PUMP still needs around 100 $ms$ to find 
a path.

%Another example is the autonomous robot arms, robot arms need to operate with 
%high precision in 
%realtime. But CPU-based motion planning has a long latency. As a result, 
%CPU-based control of robot 
%arms have to operate at very slow speed without leveraging the full operation 
%capability of the arms. 
%More powerful deployment of the motion planning algorithm needs to be used.

On-time execution of path planning is important for the safety and 
the efficiency of a vehicle. %Various efforts have been made.
Pruning \cite{pan2016fast} has been used to accelerate path planning in software.
Algorithm-specific accelerators have also been proposed
for rapid-exploring random tree (RRT) \cite{xiao2017parallel}, probablistic 
roadmap (PRM)\cite{murray2019programmable}, and 
A* \cite{kim2017brain}, using  FPGAs or 
ASICs. While 
these accelerators for path planning do address the 
individual needs in the specific scenarios, they do not target the autonomous 
driving and do not consider dynamic obstacles.

Besides, the flexibility to choose and modify the path planning algorithm to be 
accelerated  is also very important, as the 
regulations and 
algorithms are evolving continuously. However, many of the existing path 
planning accelerator designs only consider one specific algorithm \cite{xiao2017parallel} at a time with 
most of the hyper-parameters baked into the accelerator hardware at design/program time. While these 
hardwired algorithms 
do perform well and provide good performance on the targeted scenario at the time 
of 
launch, they may not be flexible enough to adapt to new or modified algorithms.
%These considerations are crucial for motion planning tasks in which a failure 
%scenario might involves 
%in severe damage or loss of human lives, such as passenger vehicle autonomous 
%driving, or robotic 
%surgeries. As a result, people can only rely on less-performant and power-efficient 
%hardware such as 
%GPU or CPU. 

% LSH
%The major complexity caused by these new concerns is the increase of 
%dimensionality. 
%Traditionally, motion planning only needs to be done in a space whose 
%dimensionality is equal to the 
%degree of freedom (DoF) of the system. For example, a point in a 2D plane has two 
%dimensions while a 
%robot arm may have different DoF depending on its number of segments. When 
%considering dynamic 
%obstacles, the time needs to be treated as an additional dimension. 

%Different predicted path of 
%obstacles, and multiple Monte-Carlo samples also add additional dimensions. 

%At a high level, motion 
%planning consists of a search step and a collision detection step. Searching in a 
%high-dimensional space 
%dramatically increases the latency.
% and application-specific solutions has been proposed to reduce the latency. 



%The increase of dimensionality of the search space not only increases the time it 
%takes to search, but 
%also increase the time it takes to do the collision checking. A single dynamic 
%obstacle will 
%manifest as multiple objects in the workspace-time space 
%\cite{schwesinger2015fast}, and in the collision 
%checking process, a path needs to be validated against all these objects, which 
%increases the collision 
%checking time as well. Even though bounding volume hierarchy (BVH) can reduce 
%the number of 
%collision checks performed, the size of the tree still increases with the additional 
%dimensionality.



%Do we also consider the programmability as a main claim????
%Another issue with today's motion planning accelerators is that many of them are 
%targeting specific 
%algorithms with application-specific implementations. However, motion planning 
%algorithm is 
%continuously 
%developing, with many new algorithms developed within the last ten or twenty 
%years %[RRT]. Car vendors 
%such as Tesla frequently update their autonomous driving software over the air. 
%Robot arm vendors may 
%also want to provide upgradability to the motion planning algorithm without 
%replacing the hardware 
%accelerator. While algorithm-specific accelerator may perform well in optimizing 
%the overall 
%performance, it lacks enough programmability and upgradability that are required 
%for today's fast 
%updated 
%software stack. 

In this paper, we address  the problem of path planning for autonomous driving with dynamic 
obstacles.
The major contributions of 
this work is as follows:


%\begin{comment}
\begin{enumerate}
\item We introduce the  space-filling curve for efficient indexing, 
memoization and pruning of the time-consuming nearest neighbor search and collision 
detection in path planning.

\item We propose a high-performance hardware implementation and a 
programming interface for memoization of the space-filling curve-indexed tree nodes, which 
is used for a nearest neighbor search  and collision detection.

\item We demonstrate that the proposed hardware-assisted approach can lead to 
significant performance improvement for path planning with dynamic obstacles in both synthetic and 
realistic benchmarks.
	
\end{enumerate}

%\end{comment}
%\begin{enumerate}
%\item We identify and propose an LSH algorithmic scheme to accelerate a general 
%motion planning 
%algorithm for both the search part and collision checking part, that is applicable to 
%a wide range of 
%motion planning algorithms;
%\item We design a hardware programmable accelerator architecture that	can 
%accommodate our 
%LSH-scheme in hardware with brings superior performance as compared to 
%existing purely 
%software-based LSH.
%\item We demonstrate the motion planning accelerator is applicable to different 
%application scenarios 
%including autonomous driving and robot arms. % with strong security and safety 
%%considerations.
%\item We compare and evaluate the accelerator with existing accelerators and 
%%%showing the superiority.
%\end{enumerate}
%To our konwledge, this is the first work that demonstrates hardware-assisted 
%memorization with Morton code for pruning exact nearest neighbor search and 
%collision detection in a sampling-based path planning, this 


==> 2020-robot-accelerator 2/prelim.tex <==
\section{Background}\label{sec:prelim}

\subsection{Sampling-based Motion Planning}
% traditional motion planning
%Traditional motion planning consists of two phases: roadmap construction 

Sampling-based motion planning algorithms such PRM 
and RRT are widely used in path planning. Compared with 
the grid-based search where the points are predefined on a grid, a sampling-based 
algorithm selects 
points by random sampling, and is more suitable for scenarios with high dimensions.
Sampling-based planning algorithm usually contains two major steps:
Nearest neighbor search and collision detection. Taking RRT as an example, RRT uses a tree 
structure to 
organize the points in the space. During the nearest neighbor search phase, a random 
point is sampled and the nearest neighbor of it in the tree is found. In the collision 
detection phase, the newly 
formed edge is checked against all obstacles to make sure that there is no collision. After 
that, it is added to the tree.
We use RRT as the baseline.



%Typically, all obstacles needs to be checked. However, the obstacles can be 
%organized 
%spatially using a hierarchy structure such as BVH \cite{yoon2006cache} so 
%that only selected obstacles need be checked with the newly formed edges.

%Another advantage of sampling-based algorithm is that it can easily be adapted to 
%include 
%probabilistic collisions and other safety-related concerns. In real-world scenario, 
%the 
%information comes from sensors and it has measurement errors. Motion planning in 
%uncertain 
%environment also depends on the predictions. 

%Besides, there are adversarial scenarios where 
%the obstacles may intentionally move in a way to increase the collision probability. 
%Sampling-based algorithm can handle these considerations by increasing the 
%number of 
%samples in different scenarios \cite{ichter2017robust}.

%One major characteristics of a sampling-based motion planning algorithm is that in 
%general, 
%the solution quality improves with increasing number of samples. 
%For high-assurance 
%applications like autonomous driving where human lives is involved, it is essential 
%to have 
%sufficient number of samples to prevent all potential hazards. CPU-based and 
%GPU-based 
%motion planning may just barely meet the need for it, and the power-efficiency is 
%not ideal. 
%Thus, people considers using hardware accelerator architecture for these 
%algorithms.

%1. collision calculation
%2. tree search
\begin{comment}

\subsection{Motion Planning Accelerators}

%In addition to the natural performance advantage of a hardware accelerator
%over a CPU, there are several other application-specific aspects why a 
%hardware motion planner make sense.

First, for a sampling-based motion planning algorithms, parallelization 
\cite{ichter2017robust,bialkowski2011massively} is natural. Motion planning algorithms performs 
search, and we can parallelize the search by using multiple workers \cite{kim2017brain}.
For hardware accelerators, these workers can be executed on multiple hardware executors.  

Second, the memory access patterns of collision detection is also suitable for a hardware 
acceleration. In collision checking process, different motion primitives needs to be checked 
against the same set of obstacles. Thus, the objects representing the obstacles will be 
stationary while the motion primitives are changing. An accelerator architecture that buffers 
the stationary objects in an on-chip memory can save a lot of memory accesses. For 
example, Dadu-p\cite{lian2018dadu} has on-chip buffers to store different obstacles. 
Other hardware acceleration techniques such as in-memory-processing  
\cite{yang2020dadu} and 
content-addressable memory \cite{yang2020accelerating} have also been proposed.

Third, some accelerator architecture uses FPGA 
\cite{murray2016microarchitecture} that directly bakes the 
obstacles in RTL logic, which significantly improves the performance.

However, the existing motion planning accelerators are targeting specific applications and are 
making application-specific specialialization  and optimizations that makes them functionally 
not intuitive to adapt to current and future needs of motion planning with higher security 
assurance. For example, Dadu-p\cite{lian2018dadu} uses an Octree structure to partition the 3D 
space, while it is suitable for robot arm, it is not suitable to represent a car in the autonomous 
driving scenario. \cite{xiao2017parallel} discusses an FPGA accelerator for RRT-star algorithm 
with static obstacles, but it is unclear how to handle dynamic obstacles with this accelerator. 
New accelerator architecture is needed to address the new concerns in motion-planning 
algorithms.

\end{comment}

\subsection{Space-filling Curves}

A space-filling curve such as a Morton curve or a Hilbert curve  \cite{sagan2012space}, 
maps a point in a 
high-dimensional space onto a 1D curve while probabilistically maintaining the 
proximity. This means that if two points  are close to each other on the mapped 
curve, 
then they will also be close to each other in the original high 
dimensional space with high probability. 
This property can be used to efficiently index the points. If the Morton 
codes of two points only differ in the least significant bit, then 
with high probability they are nearest neighbors. 
%If there exist obstacles whose Morton code is close to that of a node, then it is 
%likely that there is a collision  that node.
We use the Morton code to index the nodes in the tree.

\subsection{Content-Addressable Search}

Sampling-based planning involves finding nearest neighbors and collision 
detection. Both can be implemented using an $O(n)$ algorithm where $n$ is the 
number of nodes or obstacles. To reduce the computation complexity, a tree-based 
structure such as bounding volume hierarchy \cite{schwesinger2015fast} or kd-tree has 
been 
used, which can reduce the 
complexity to $O(log\; n)$. However, for large number of obstacles and an increasing number of
nodes, tree-based algorithms still take non-trivial amount of time. On the other hand, 
content-addressable
search provides $O(1)$ complexity to these problems. Content-addressable memory 
has been 
used in caches and load/store queues in microprocessors. It has also been used in the 
path planning scenario \cite{yang2020accelerating} to store all nodes and obstacles. 
In this paper, we use the associative memory as a cache to keep most 
recent checked nodes.


\subsection{Pruning in Path Planning}

An exact nearest neighbor search or collision detection is time-consuming. Early 
decision without going through an exact algorithm is key to reduce the overall 
execution time. In~\cite{pan2011fast}, a fast location-sensitive hash method that 
calculates the collision probability has been used to pruning exact collision 
detection for cases with very high or very low  probability of collision in sampling-based 
algorithm. In this work, we also use pruning 
to accelerate the path planning.





==> 2020-robot-accelerator 2/related_work.tex <==



%\begin{comment}

\section{Related Work}\label{sec:related_work}

%\subsection{Motion Planning Algorithms}


\begin{comment}}
\subsection{Planning with Dynamic Obstacles}

Dynamic obstacles complicate the planning problem and there are different ways to 
handle them.
The most straightforward way is to plan without considering dynamic obstacles and 
do replanning if there is a collision with dynamic obstacles
\cite{vemula2016path,van2006anytime}. There are also methods based on the 
probability distribution of the dynamic obstacles, such as in 
\cite{kushleyev2009time,hardy2013contingency}.
In \cite{phillips2011sipp},  the time domain of the path planning problem with 
dynamic obstacles is divided into several ``safe intervals'' and perform path planning 
with static obstacles inside the intervals. Unlike these studies which still perform 
planning in the original space with same dimension, we treat time as an additional 
dimension.

\end{comment}



\begin{comment}
\subsection{Software Planning Acceleration}

Since planning with dynamic obstacles is time-consuming, acceleration is important.
 Pan et al. \cite{pan2016fast} use location sensitive hash 
(LSH) for pruning exact collision detection computation for acceleration. In this paper, 
we also use a similar 
pruning approach.
However, our work differs in several 
ways from the LSH method. 
First, we focus on an autonomous driving scenario, which usually only has 
limited degrees of 
freedom. In this case, the benefit of using multiple hash functions to reduce 
the dimension is 
marginal.
Instead, we use the space-filling curve. However, precise matching of  
Morton code is 
difficult, and we remove some LSBs and only use MSBs  
of the Morton code in order to increase the probability of a Morton 
store hit.
Using one table instead of multiple LSHs also makes an efficient hardware 
implementation possible. 

%These methods accelerate path planning with 
%dynamic obstacles, but may still not meet fit the real-time requirement only with 
%software implementation. In this work, we propose hardware-based acceleration 
%approach to deal with dynamic obstacles.


%Dynamic obstacles are a source of uncertainty in path planning.
%% planning under uncertainty
%There are several existing work on path planning that takes into account 
%some of the uncertainties. For example \cite{agha2014firm} formulates it as 
%an partially-observable Markov Decision Process (POMDP). 
%\cite{prentice2009belief} consider the uncertainty in vehicle 
%localization 
%and use belief roadmap for path planning, while \cite{artunedo2020motion} 
%perform planning on occupancy grid.\cite{janson2018monte} uses 
%Monte-Carlo simulation for dealing with uncertainties of localization and 
%calculates the corresponding collision probability.  
%\cite{nakhaei2008framework} 
%considers uncertainty in the map and use Monte-Carlo algorithm to 
%evaluate collision probability during planning. \cite{kushleyev2009time} 
%considers dynamic obstacles, since the distribution of dynamic obstacles 
%will dissipate over time, a time limit which the dynamic obstacles can be 
%ignored is derived. \cite{hardy2013contingency} considers dynamic 
%obstacles that may have multiple path to choose but they will have 
%common segments, the algorithm minimizes the collision probability with 
%the common segments. 

%\cite{agha2014firm,prentice2009belief,artunedo2020motion,nakhaei2008framework}
%\cite{hardy2013contingency,kushleyev2009time}

%%mcts planning
%Monte-Carlo tree search is a promising algorithm to deal with uncertainties 
%especially in gaming. There are some existing works that apply MCTS in the 
%planning problems. \cite{best2019dec} uses MCTS for multi-robot 
%planning. \cite{van2013guided} uses MCTS for planning of events. 
%\cite{hyatt2020versatile} uses MCTS to perform coverage planning. 
%\cite{kurzer2018decentralized} uses MCTS for decentralized cooperative 
%planning.
%\cite{best2019dec,janson2018monte,van2013guided,janson2018safe,hyatt2020versatile,bry2011rapidly}
% mcts accelerator
%There has been some accelerator architecture proposed for MCTS. For 
%example, \cite{qasemi2014highly} proposed an FPGA-based MCTS 
%accelerator built for Blokus game. \cite{graf2011parallel} build a similar 
%accelerator for Go. 

\end{comment}


\begin{comment}
\subsection{Hardware Planning Accelerations}
\end{comment}

There are multiple
previous studies on hardware planning accelerators. 
For example, Murray et al.\cite{murray2016microarchitecture} 
propose an accelerator for motion planning for robot arms. 
Using an ASIC, Lian et al.\cite{lian2018dadu} create a motion planning accelerator based on octree 
where 
the 
map can be updated according to the environment. 
%Di et al.\cite{di2015energy} provide an accelerator for UAV coverage planning.  
A hybrid RRT architecture is proposed in 
\cite{malik2016fpga} and implemented in FPGA. In \cite{xiao2017parallel} 
an FPGA accelerator for RRT* is implemented.  
%There are also planning based on A* search on grid 
%\cite{kim2017brain}. 
%Apart from FPGA or ASIC-based accelerators, there are also GPU-based 
%algorithms that leverage the massive-parallel nature of the algorithms
%\cite{ichter2017robust}.
Unlike an accelerator or a customized processor, our approach is based on 
hardware-based memoization as ISA extension.


The content-addressable memory for path planning is also used in 
\cite{yang2020accelerating}. However, our work is different from it in several ways. 
First, our work has just one 
unified Morton store that is used  for both collision detection and nearest neighbor 
search, while 
the previous work uses 
two separate stores. Second, our work is designed as an ISA extension to a 
normal processor, 
and adapt to 
different algorithms, while the previous work \cite{yang2020accelerating} is limited
to a fixed algorithm with the size of 
the 
problem that can 
fit into the ternary-CAM available on chip. 
Kim et. al. \cite{kim2017brain} also uses CAM for path planning algorithms. 
However, it only targets the A* search algorithm, not sampling-based path 
planning. 
Also, the previous work cannot completely 
skip the tree search and does not explicitly accelerate collision detection.
Table~\ref{tab:compare} summarizes 
the major differences between our work and the related work on pruning and 
CAM-based acceleration. 


% other accelerator
%There are also accelerator for robotic tasks other than motion planning.
%\cite{amundsen2019finger} provides an accelerator for peak detection. 
 %\cite{suleiman2019navion} provides an accelerator for sensor fusion.
 

%\cite{murray2016microarchitecture,xu2019tigris,qasemi2014highly}
%\cite{chinnaaiah2015fpga,di2015energy,kurzer2018decentralized,ichter2017robust,amundsen2019finger}
%\cite{li2019fpga,murray2019programmable,zhang2019efficient,suleiman2018energy}
%\cite{xiao2017parallel,kuffner2000rrt,malik2016fpga,kim201614,kim2017brain}
%\cite{leng2019asymmetric,suleiman2019navion,lian2018dadu,everson20192,honkote20192}
%\cite{ichter2017robust}


%\end{comment}


==> discussion.tex <==
\section{Discussion}\label{sec:discussion}



Our approach is inspired by two key ideas: pruning, and content-addressable 
memory-based acceleration.
Pruning is inspired by Pan\cite{pan2016fast}, which uses location sensitive hash 
(LSH) for pruning exact collision detection computation. 
However, the proposed software optimization with the Morton codes differs in several 
ways. 
First, we are focusing on autonomous driving scenario, which usually only have 
limited degrees of 
freedom, in these case, the benefit of using multiple hash functions to reduce 
the dimension is 
marginal.
Instead, we use the space-filling curve. However, in this case, precise matching of  
Morton code is 
hard, and we remove some LSBs and only use MSBs  
of the Morton code in order to increase the probability of a Morton 
store hit.
Using one table instead of multiple LSHs also makes an efficient hardware implementation possible. 

 \begin{table*}[h]
%	\footnotesize
\centering
\scriptsize
%\footnotesize
	\caption{Comparison with existing works.}\label{tab:compare}
	\begin{tabular}{|l|| l|l|l|l|l|l| l|}
		\hline
		work &  implementation & encode  &  reported improvement  & 
		algorithm & dynamic &accelerate& accelerate\\ 
		& & & over SW& flexibility& obstacles &tree search& collision detection\\ \hline\hline
		\cite{pan2016fast} &  software & LSH  & 1.46X   &  yes& no & no& yes \\ \hline
		\cite{yang2020accelerating} & accelerator & RENE \cite{bremler2018encoding}  &  
		235X&  no& no &yes&yes \\ \hline
		 \cite{kim2017brain} & processor & Zobrist \cite{zobrist1990new} & 8.63X & 
		 no & 
		 no&yes& no\\ \hline
		this work &  ISA extension &   Morton & 8X &  yes &yes&yes&yes\\ \hline
	\end{tabular}
    \label{tab:comparion}
	\vspace{-0.5cm}
\end{table*}

 The content-addressable memory for path planning is inspired by 
 \cite{yang2020accelerating}. However, our work is different from it in several ways. 
 First, our work has just one 
 unified Morton store that is used  for both collision detection and nearest neighbor 
 search, while 
 the previous work uses 
 two separate stores. Second, our work is designed as an ISA extension to a 
 normal processor, 
 and adapt to 
 different algorithms, while the previous work \cite{yang2020accelerating} is limited
 to a fixed algorithm with the size of 
 the 
 problem that can 
 fit into the ternary-CAM available on chip. 
 \cite{kim2017brain} also uses CAM for path planning algorithms. 
 However, the it only targets the A* search algorithm, not sampling-based path 
 planning. 
 Also, this previous work cannot completely 
 skip the tree search and does not explicitly accelerate collision detection.
 Table~\ref{tab:compare} summarizes 
 the major differences between our work and the related work on pruning and CAM-based acceleration. 
% Our work strikes a 
% good balance in performance and flexibility.
 
 

 
 
 
\begin{comment}

\subsection{Location Sensitive Hash}

As mentioned, new concerns in motion planning problems, including dynamic 
obstacles, 
multiple paths of obstacles, and probabilistic collision \cite{hardy2013contingency}, 
have 
significantly increase the dimensionality and the number of samples in a 
sampling-based 
motion planning algorithms. LSH-based method \cite{pan2016fast} is an effective 
way to 
accelerate the 
search in high-dimensional space. Usually, LSH have multiple hashtables with 
different hash 
functions. Points that are close to each other are likely to be mapped to the same 
bucket in 
one or more hashTables. LSH is efficient in search for the nearest neighbors, which 
is needed 
for a sampling-based motion planning algorithm like RRT \cite{guo2018foggycache}. 
LSH 
has also been used for collision checking in motion-planning algorithms 
\cite{pan2011fast} on the assumption that collision checking takes most of 
	the 
computation time in motion planning. LSH is a good primitive for accelerating motion 
planning algorithms.



\subsection{Existing LSH Scheme}

Though LSH has been used with existing motion planning for nearest neighbor 
search or 
collision detection in software. Only modest improvement has been observed 
because unoptimized 
hash table may consume significant hardware resource. Hash table can be 
hardware friendly since on-chip memory like caches can be used to accelerate the 
table 
lookup by preventing direct access to the main memory similar to how translation 
lookup 
buffer can help accelerating pagetable lookup. However, on-chip memory has 
limited sizes 
that might not be able to cache the entire table and it remains unclear what is the 
proper size 
of the caches.  Even though there are existing works on building cache-friendly 
motion 
planning algorithms, there have not been any works on software-hardware 
co-optimized 
LSH. 

%LSH only accelerates collision checking, but with increased dimensions, tree 
%traversal is also important

% existing LSH does not leverage the HW 


Location sensitive hash (LSH) can reduce the computation time in a high dimensional 
space [cite]. LSH is a class of hash function that maps spatially remote coordinates 
to hash values with larger distances. A formal definition of LSH can be found at 
[cite]. Using LSH, similar queries (searches) in the high dimensional space can be 
accessed quickly by directly looking up the hash table which stores queries with 
similar LSH values. LSH has also been used separately for collision detection in the 
path planning algorithm, with the assumption that in traditional path planning 
algorithm, collision checking, rather than tree traversal takes most of the time. 
However, in high dimensional case with more obstacles, and when we apply BVH to 
prune unnecessary collision checkings, we observe that the collision checking and 
tree traversal are equally important in the computation time. 
%An LSH-based scheme that accelerates both collision checking and tree traversal 
%is needed in these 
%scenarios.
Besides, most of the existing LSH-based scheme are purely software-based 
\cite{pan2011fast} without 
leveraging hardware structures that could be used in a accelerator structure. As a 
result, existing 
approach \cite{pan2016fast} for accelerating collision checking only bring about less 
than 30\% 
performance improvement. 

\end{comment}


==> implementation.tex <==
%\section{Implementation}\label{sec:implemenation}

==> prelim.tex <==
\section{Background}\label{sec:prelim}

\subsection{Sampling-based Motion Planning}
% traditional motion planning
%Traditional motion planning consists of two phases: roadmap construction 

Sampling-based motion planning algorithms such PRM 
and RRT are widely used in path planning. Compared with 
the grid-based search where the points are predefined on a grid, a sampling-based 
algorithm selects 
points by random sampling, and is more suitable for scenarios with high dimensions.
Sampling-based planning algorithm usually contains two major steps:
Nearest neighbor search and collision detection. Taking RRT as an example, RRT uses a tree 
structure to 
organize the points in the space. During the nearest neighbor search phase, a random 
point is sampled and the nearest neighbor of it in the tree is found. In the collision 
detection phase, the newly 
formed edge is checked against all obstacles to make sure that there is no collision. After 
that, it is added to the tree.
We use RRT as the baseline.



%Typically, all obstacles needs to be checked. However, the obstacles can be 
%organized 
%spatially using a hierarchy structure such as BVH \cite{yoon2006cache} so 
%that only selected obstacles need be checked with the newly formed edges.

%Another advantage of sampling-based algorithm is that it can easily be adapted to 
%include 
%probabilistic collisions and other safety-related concerns. In real-world scenario, 
%the 
%information comes from sensors and it has measurement errors. Motion planning in 
%uncertain 
%environment also depends on the predictions. 

%Besides, there are adversarial scenarios where 
%the obstacles may intentionally move in a way to increase the collision probability. 
%Sampling-based algorithm can handle these considerations by increasing the 
%number of 
%samples in different scenarios \cite{ichter2017robust}.

%One major characteristics of a sampling-based motion planning algorithm is that in 
%general, 
%the solution quality improves with increasing number of samples. 
%For high-assurance 
%applications like autonomous driving where human lives is involved, it is essential 
%to have 
%sufficient number of samples to prevent all potential hazards. CPU-based and 
%GPU-based 
%motion planning may just barely meet the need for it, and the power-efficiency is 
%not ideal. 
%Thus, people considers using hardware accelerator architecture for these 
%algorithms.

%1. collision calculation
%2. tree search
\begin{comment}

\subsection{Motion Planning Accelerators}

%In addition to the natural performance advantage of a hardware accelerator
%over a CPU, there are several other application-specific aspects why a 
%hardware motion planner make sense.

First, for a sampling-based motion planning algorithms, parallelization 
\cite{ichter2017robust,bialkowski2011massively} is natural. Motion planning algorithms performs 
search, and we can parallelize the search by using multiple workers \cite{kim2017brain}.
For hardware accelerators, these workers can be executed on multiple hardware executors.  

Second, the memory access patterns of collision detection is also suitable for a hardware 
acceleration. In collision checking process, different motion primitives needs to be checked 
against the same set of obstacles. Thus, the objects representing the obstacles will be 
stationary while the motion primitives are changing. An accelerator architecture that buffers 
the stationary objects in an on-chip memory can save a lot of memory accesses. For 
example, Dadu-p\cite{lian2018dadu} has on-chip buffers to store different obstacles. 
Other hardware acceleration techniques such as in-memory-processing  
\cite{yang2020dadu} and 
content-addressable memory \cite{yang2020accelerating} have also been proposed.

Third, some accelerator architecture uses FPGA 
\cite{murray2016microarchitecture} that directly bakes the 
obstacles in RTL logic, which significantly improves the performance.

However, the existing motion planning accelerators are targeting specific applications and are 
making application-specific specialialization  and optimizations that makes them functionally 
not intuitive to adapt to current and future needs of motion planning with higher security 
assurance. For example, Dadu-p\cite{lian2018dadu} uses an Octree structure to partition the 3D 
space, while it is suitable for robot arm, it is not suitable to represent a car in the autonomous 
driving scenario. \cite{xiao2017parallel} discusses an FPGA accelerator for RRT-star algorithm 
with static obstacles, but it is unclear how to handle dynamic obstacles with this accelerator. 
New accelerator architecture is needed to address the new concerns in motion-planning 
algorithms.

\end{comment}

\subsection{Space-filling Curves}

A space-filling curve such as a Morton curve or a Hilbert curve  \cite{sagan2012space}, 
maps a point in a 
high-dimensional space onto a 1D curve while probabilistically maintaining the 
proximity. This means that if two points  are close to each other on the mapped 
curve, 
then they will also be close to each other in the original high 
dimensional space with high probability. 
This property can be used to efficiently index the points. If the Morton 
codes of two points only differ in the least significant bit, then 
with high probability they are nearest neighbors. 
%If there exist obstacles whose Morton code is close to that of a node, then it is 
%likely that there is a collision  that node.
We use the Morton code to index the nodes in the tree.

\subsection{Content-Addressable Search}

Sampling-based planning involves finding nearest neighbors and collision 
detection. Both can be implemented using an $O(n)$ algorithm where $n$ is the 
number of nodes or obstacles. To reduce the computation complexity, a tree-based 
structure such as bounding volume hierarchy \cite{schwesinger2015fast} or kd-tree has 
been 
used, which can reduce the 
complexity to $O(log\; n)$. However, for large number of obstacles and an increasing number of
nodes, tree-based algorithms still take non-trivial amount of time. On the other hand, 
content-addressable
search provides $O(1)$ complexity to these problems. Content-addressable memory 
has been 
used in caches and load/store queues in microprocessors. It has also been used in the 
path planning scenario \cite{yang2020accelerating} to store all nodes and obstacles. 
In this paper, we use the associative memory as a cache to keep most 
recent checked nodes.


\subsection{Pruning in Path Planning}

An exact nearest neighbor search or collision detection is time-consuming. Early 
decision without going through an exact algorithm is key to reduce the overall 
execution time. In~\cite{pan2011fast}, a fast location-sensitive hash method that 
calculates the collision probability has been used to pruning exact collision 
detection for cases with very high or very low  probability of collision in sampling-based 
algorithm. In this work, we also use pruning 
to accelerate the path planning.




